An embedding for EEG signals learned using a triplet loss

Neurophysiological time series recordings like the electroencephalogram (EEG) or local field potentials are obtained from multiple sensors. They can be decoded by machine learning models in order to estimate the ongoing brain state of a patient or healthy user. In a brain-computer interface (BCI), this decoded brain state information can be used with minimal time delay to either control an application, e.g., for communication or for rehabilitation after stroke, or to passively monitor the ongoing brain state of the subject, e.g., in a demanding work environment. A specific challenge in such decoding tasks is posed by the small dataset sizes in BCI compared to other domains of machine learning like computer vision or natural language processing. A possibility to tackle classification or regression problems in BCI despite small training data sets is through transfer learning, which utilizes data from other sessions, subjects or even datasets to train a model. In this exploratory study, we propose novel domain-specific embeddings for neurophysiological data. Our approach is based on metric learning and builds upon the recently proposed ladder loss. Using embeddings allowed us to benefit, both from the good generalisation abilities and robustness of deep learning and from the fast training of classical machine learning models for subject-specific calibration. In offline analyses using EEG data of 14 subjects, we tested the embeddings' feasibility and compared their efficiency with state-of-the-art deep learning models and conventional machine learning pipelines. In summary, we propose the use of metric learning to obtain pre-trained embeddings of EEG-BCI data as a means to incorporate domain knowledge and to reach competitive performance on novel subjects with minimal calibration requirements.

==> content_report/electromag.tex <==
\newcommand{\elec}{\mathbf{E}}
\newcommand{\magn}{\mathbf{B}}
\newcommand{\normal}{\mathbf{n}}
\newcommand{\current}{\mathbf{J}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\section{Electromagnetic Reminders}\label{app:electromag}
\subsection{Maxwell's equations}

\begin{table}[h]
%\centering
\begin{tabular}{|l|l|l|}
    \hline
    Name &  Local form & Integral form \\ \hline
    Gauss's law & $\nabla\cdot \elec = \frac{\rho}{\epsilon_0}$
        & $\oiint_{\partial\Omega}\elec\cdot\normal ds = \iiint_\Omega\frac{\rho}{\epsilon_0}d\mathbf{r}$ \\ \hline
    Gauss's law for magnetism & $\nabla \cdot\magn = 0$
        & $\oiint_{\partial\Omega}\magn\cdot\normal ds = 0$ \\ \hline
    Faraday's law & $\nabla\times\elec=-\frac{\partial\magn}{\partial t}$
        & $\oint_{\partial S}\elec\cdot\overrightarrow{dl} = -\iint_S\frac{\partial\magn}{\partial t}ds$ \\ \hline
    Ampère's circuital law
        & $\nabla\times\magn = \mu_0\left(\current+\epsilon_0\frac{\partial\elec}{\partial t}\right)$
        & $\oint_{\partial S}\magn\cdot\overrightarrow{dl} = \mu_0\iint_S\left(\current+\epsilon_0\frac{\partial\elec}{\partial t}\right)\cdot\normal ds$ \\ \hline
\end{tabular}
\caption[Maxwell's equations]{Maxwell's equations.

With the following constants :
$\epsilon_0=8.85\cdot10^{-12}kg^{-1}m^{-3}A^2s^4$,
$\mu_0=4\pi10^{-7}kg m A^{-2}s^{-2}$
and $\epsilon_0\mu_0 c^2=1$.

$\elec$ is expressed in $Vm^{-1}$, $\magn$ in $T$ (tesla), $\current$ in $Am^{-2}$ and $\rho$ in $Cm^{-3}$.

$\nabla\cdot$ is the divergence operator and $\nabla\times$ is the curl operator.
$\oiint_{\partial\Omega}$ is a surface integral over the closed surface $\partial\Omega$,
$\iiint_\Omega$ is a volume integral over the volume $\Omega$,
$\oint_{\partial S}$ is a line integral over the closed boundary curve $\partial S$ and
$\iint_{S}$ is a surface integral over the surface $S$.}
\label{tab:maxwell_eq}
\end{table}


Gauss's law links the electric field to the electric charges that cause it.\\
Gauss's law for magnetism states that the magnetic flux through a closed surface is always null.\\
Faraday's law describes how a time varying magnetic field induces an electric field.\\
Ampère's circuital law states that magnetic fields can be generated by electric current and by time varying electric fields~\cite{clerc2010inverse}.


\subsection{Stationary or quasi-static case}
A quasi-static approximation refer to the idea that the sources in the problem change sufficiently slowly
so that the system can be considered at equilibrium at all times.
In electromagnetism, such an approximation is made
if we consider that the time derivatives can be neglected compared to other quantities.
If we make this approximation, the equations can be simplified


\begin{table}[h]
\centering
\begin{tabular}{|l|l|}
    \hline
    Name &  Local form \\ \hline
    Faraday's law in electro-quasistatic regime & $\nabla\times\elec=0$
\\ \hline
    Ampère's circuital law  in magneto-quasistatic regime
        & $\nabla\times\magn = \mu_0\current$
\\ \hline
\end{tabular}
\caption[Maxwell's equations in quasi-static regime]{Maxwell's equations in quasi-static regime}
\label{tab:maxwell_eq_static}
\end{table}

A consequence of the time-invariant Maxwell-Faraday equation
is that $\elec$ now  derives from the electrical potential:
\begin{align}
    \elec = -\nabla V
\end{align}


==> content_report/neuro_and_bci.tex <==
% \let\textcircled=\pgftextcircled

\chapter{Neurophyiology and BCI paradigms}
\label{chap:prereq}
This chapter is dedicated to the introduction of the medical knowledge needed to understand and motivate the work performed.
We will first talk about the electrical activity of the brain.
Then, we will consider how it can be detected and recorded
and finally, we will present \acrlong{bci}s.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Electromagnetic Prerequisites}
% \subsection{Maxwell's equations}
% \begin{tabular}{|l|l|l|}
%     \hline
%     Name &  Local form & Integral form \\ \hline
%     Gauss's law & $\nabla\cdot \elec = \frac{\rho}{\epsilon_0}$
%         & $\oiint_{\partial\Omega}\elec\cdot\normal ds = \iiint_\Omega\frac{\rho}{\epsilon_0}d\mathbf{r}$ \\ \hline
%     Gauss's law for magnetism & $\nabla \cdot\magn = 0$
%         & $\oiint_{\partial\Omega}\magn\cdot\normal ds = 0$ \\ \hline
%     Faraday's law & $\nabla\times\elec=-\frac{\partial\magn}{\partial t}$
%         & $\oint_{\partial S}\elec\cdot\overrightarrow{dl} = -\iint_S\frac{\partial\magn}{\partial t}ds$ \\ \hline
%     Ampère's circuital law
%         & $\nabla\times\magn = \mu_0\left(\current+\epsilon_0\frac{\partial\elec}{\partial t}\right)$
%         & $\oint_{\partial S}\magn\cdot\overrightarrow{dl} = \mu_0\iint_S\left(\current+\epsilon_0\frac{\partial\elec}{\partial t}\right)\cdot\normal ds$ \\ \hline
% \end{tabular}

% With the following constants :
% $\epsilon_0=8.85\cdot10^{-12}kg^{-1}m^{-3}A^2s^4$,
% $\mu_0=4\pi10^{-7}kg m A^{-2}s^{-2}$\\
% and $\epsilon_0\mu_0 c^2=1$.\\
% $\elec$ is expressed in $Vm^{-1}$, $\magn$ in $T$ (tesla), $\current$ in $Am^{-2}$ and $\rho$ in $Cm^{-3}$.\\
% $\nabla\cdot$ is the divergence operator and $\nabla\times$ is the curl operator.
% $\oiint_{\partial\Omega}$ is a surface integral over the closed surface $\partial\Omega$,
% $\iiint_\Omega$ is a volume integral over the volume $\Omega$,
% $\oint_{\partial S}$ is a line integral over the closed boundary curve $\partial S$ and
% $\iint_{S}$ is a surface integral over the surface $S$.\\

% Gauss's law links the electric field to the electric charges that cause it.\\
% Gauss's law for magnetism states that the magnetic flux through a closed surface is always null.\\
% Faraday's law describes how a time varying magnetic field induces an electric field.\\
% Ampère's circuital law states that magnetic fields can be generated by electric current and by time varying electric fields.


% \subsection{Stationary or quasi-static case}
% A quasi-static approximation refer to the idea that the sources in the problem change sufficiently slowly
% such that she system can be considered at equilibrium at all times.
% In electromagnetism, such an approximation is made
% if we consider that the time derivatives can be neglected compared to other quantities.
% If we make this approximation, the equations can be simplified




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Brain Electrical Activity}

This section is focused on electrophysiology of the human brain.
The brain is the most complex known biological structure~\cite{shepherd1994neurobiology}.
It is estimated to contain around 100 billion neurons~\cite{azevedo2009equal} organized in a network.

\subsection{Brain's elementary electrical activity}
A neuron is a cell that possess in particular several \textbf{dendrites} and one \textbf{axon}
(a neuron representation is in Figure~\ref{fig:neuron}).
Dendrites can be seen as \textit{inputs} of neurons and axons as \textit{outputs}.
An axon has multiple terminals and they are connected to other neurons via their \textbf{synapses}.
As other cells, neurons possess a membrane, relatively permeable to ions, that separate the inside and the outside of the cell.
The ion concentration difference between intra and extracellular compartments generate
a chemical gradient that makes ions move to the less concentrated compartment.
% But the resting electrical potential push them towards (or keeps them at)
% the compartment with opposite charge.
Moreover, the membrane electrical potential push them towards (or keeps them at)
a certain compartment depending on the ion equilibrium potential
(given by Nernst equation that we will not address in this document).
This combination is called the electrochemical gradient
and will define the way each ion will spontaneously move.
The ion concentration difference between the sides of the membrane makes it \textbf{polarized}.

To communicate, neurons liberate neurotransmitters through their synapses.
They induce the opening of ion channels on the receiving neuron's membrane,
which allow the passage of ions in the direction of the electrochemical gradient.
This electric charge flow induces a current (see electromagnetism reminders in Appendix~\ref{app:electromag}).
This event is called a \textbf{\acrfull{psp}}.
Depending on the type of ion channels opened,
some decrease the polarisation of the membranes (excitatory \acrshort{psp})
and some increase it (inhibitory \acrshort{psp}).
If the depolarisation exceed a certain threshold,
sodium voltage-gated ion channels are opened and
a current travels along the axon.
This current is called an \textbf{\acrfull{ap}}.
\acrshort{ap}s have an \textit{all or nothing} behavior with a current that has always the same amplitude,
in contrast to \acrshort{psp}s that have graduated response depending on the amount of recruited channels
~\cite{clerc2016brain, maksymenko2019novel, hitziger2015modeling, clerc2010inverse}.

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{illustrations/neuron.png}
    \caption[Neuron]{Schematic representation of a neuron. Source~\cite{maksymenko2019novel}.}
    \label{fig:neuron}
\end{figure}

\subsection{Physical quantities}\label{sec:quantities}
A typical \acrshort{ap} lasts between 1 and 3 ms and has an amplitude of 100 mV.
A \acrshort{psp} will last around 20 ms. Their amplitude is variable and lower than \acrshort{ap}'s, around 10 mV.
These dipoles participate to the generation of the electro-magnetic field
(electro-magnetic reminders in appendix~\ref{app:electromag})
but very weakly.
To have a significant impact on the field, an event (\acrshort{ap} or \acrshort{psp})
must occur relatively simultaneously to other events.
We observe that most of the electrical field generated by the brain is caused by \acrshort{psp}s.
They tend to sum up better together than \acrshort{ap}s due to their duration and
the amplitude difference is not the predominant parameter at stake here.
A typical \acrshort{psp} is similar to a 20~fAm current dipole.
The current recording techniques (see section~\ref{sec:rec_brain})
would only allow the detection of the field generated by, at least, a 10~nAm curent dipole
from outside the head.
This means that about a million of simultaneously active synapses are required
to be detectable.

Also, given the size of the head and the time scale of the observed events (a few milliseconds),
first, the quasi-static approximation can be applied to the Maxwell equations
and thus, the electric and magnetic fields can be considered uncoupled.
Second, considering also the propagation speed of electro-magnetic waves
(around $3\cdot 10^8\text{ m/s}$ in a vacuum)
and the quasi-static approximation again, it can be considered that
an emitting source in the brain will be perceived without delay and simultaneously from all
points at the surface of the head.
Moreover, multiple sources are assumed to add up linearly
when they are sensed by the same sensor.
For more details, please refer to~\cite{clerc2016brain, clerc2010inverse}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Recording the brain activity}\label{sec:rec_brain}
There are many different methods to observe brain activity.
Each of them is able to report a certain aspect of this activity.
But none, even combined, is able to exhaustively give functional brain recordings at the neuron level yet.
We will present in details \acrshort{eeg} and \acrshort{meg} and then list some other methods.

\subsection{EEG}
\acrshort{eeg} stands for \textbf{\acrlong{eeg}}.
This method allows us to observe the brain through it's electrical activity.
It uses electrodes placed at the surface of the scalp that keep track of electrical potentials.
An \acrshort{eeg} cap is shown in Figure~\ref{fig:cap} left.
\acrshort{eeg} has a very low spatial resolution.
\acrshort{eeg} caps can contain up to 256 electrodes,
and if sources' locations are needed then an inverse problem has to be solved.
But it has a very good temporal resolution, sampling rates can go exceed 2000~Hz,
and because of the propagation speed of the electro-magnetic waves,
\acrshort{eeg} can be considered as a true real-time observation method of the brain
as opposed to fMRI for example.
When a brain source emits a signal, it is seen without significant delay on all the sensors
(c.f. section~\ref{sec:quantities}) and
the amplitudes at which it is perceived by the sensors depend on the electrical conductivities
of the different layers crossed by the wave.
\acrshort{eeg} is also cheap relative to other brain observation methods.

Due to the amplitude of the signal of interest, \acrshort{eeg} is very sensible to perturbations.
The 50/60~Hz electrical current is visible on recordings and has to be notch-filtered.
Muscle contractions, mastication, eye blinks, swallowing
and many other sources can also produce artefacts.

It is also possible, in the case of severe epilepsy, to surgically place the electrodes
directly at the surface of the exposed brain or even inside of it.
We then talk about \textbf{\acrfull{ecog}}
or \textbf{\acrfull{ieeg}}.
It has the advantage of not having the skull in the way blocking the signal.
The skull has a low electrical conductivity. It also brings the electrodes closer to the sources
(potential decreases with the squared distance to the source).

% {\huge\itshape TODO: EEG RECORDING }

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{illustrations/eeg_helmet.png}
    \caption[\acrshort{eeg} cap and scalp potential]
    {\textbf{Left}: \acrshort{eeg} recording session with multi-electrode cap
    at Inria Sophia Antipolis, source~\cite{hitziger2015modeling}.
    \textbf{Right}: Visualization of potential differences on the scalp, source~\cite{vallaghe2008modelisation}}
    \label{fig:cap}
\end{figure}

\subsection{MEG}
\textbf{\acrfull{meg}} detects the magnetic fields
produced by the brain electrical activity.
So the type of activity recorded by \acrshort{meg} is the same as \acrshort{eeg} but, as opposed to the latter,
\acrshort{meg} is rather independent of head geometry because magnetic fields
are not affected by electrical conductivity
(though ferromagnetic implants would affect it and are hereby prohibited).
The amplitude at which a source is perceived by a sensor only depends on the distance between them.
See appendix~\ref{app:electromag} for more details.
It has a temporal resolution similar to \acrshort{eeg} and possibly a better spatial one.
But the equipment involved is heavier (see Figure~\ref{fig:meg_room})
and much more costly (including a magnetically shielded room).

\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{illustrations/meg_setup.jpg}
    \caption[Person undergoing a MEG]{Person undergoing a \acrshort{meg}. Source~\cite{wiki:Magnetoencephalography}}
    \label{fig:meg_room}
\end{figure}
% {\huge \itshape TODO: image MEG}

\subsection{Other methods}
There exists other methods to record brain activity that do not rely on its electrical activity.
\begin{itemize}
    \item \textbf{\acrfull{fmri}} is exploiting the hypothesis
    that active parts of the brain have a higher oxygen consumption than passive ones.
    \item \textbf{\acrfull{pet}} uses radioactive markers.
    They are chosen to fix themselves on molecules consumed by active areas of the brain.
    \item \textbf{\acrfull{spect}} is similar to \acrshort{pet}
    but uses gamma ray emitters as radioactive markers.
    \item \textbf{\acrfull{lm}} can be used to visualize single neurons.
    \item \textbf{\acrfull{em}} is the only modality so fare able to image individual synapses.
\end{itemize}
Figure~\ref{fig:resolution_graph} presents the different existing techniques according to their spatial and temporal resolutions.

\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{illustrations/spatio_temporal_resolution.png}
    \caption[Temporal and spatial resolutions of brain imaging methods]
    {Different brain imaging modalities and their spatial and temporal resolutions. Source~\cite{pfister2014visualization}}
    \label{fig:resolution_graph}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Brain-Computer Interfaces} \label{sec:BCI}

A \textbf{\acrfull{bci}} is a direct communication interface
between a brain and an external device.
In most \acrshort{bci} systems reported in the literature,
the brain activity is recorded through an \acrshort{eeg} cap
for their responsiveness (allowing real-time observation)
and their quite limited cost. \acrshort{meg} and \acrshort{fmri} have also been used in some cases.
Below, some brain computer interface paradigms are presented.

\subsection{Mental Imagery tasks}

\textbf{Mental image} refers to representations and the accompanying experience of sensory information without a direct external stimulus~\cite{kosslyn2005mental,pearson2015mental}.
For example, a subject can use his imagination or memory to get a mental image
of a bird when none is within sight.
He will then be able to \textit{see} it's shape, color, texture, and so on, but not through his eyes.

\textbf{Mental imagery-based \acrshort{bci}s}
allow users to send commands to computers by performing mental-imagery tasks.
A list of mental images is defined and a command is associated to each of them.
For example, the mental image \textit{left hand} can be linked to \texttt{command\_1}
and \textit{right hand} to \texttt{command\_2}
so whenever the user "thinks" about
his left hand, the \texttt{command\_1} is executed.
In Figure~\ref{fig:cybathlon}, we can see a subject
training to command an avatar to move left and right using mental imagery-based \acrshort{bci}
to participate to the cybathlon
(an international competition for disabled competitors
using technical assistance systems).

One of the challenges in mental imagery-based \acrshort{bci}
is to find appropriate mental images.
They have to suite the user: even after long sessions,
he must still be able to produce a clear mental image.
He might have more affinities with some than with others.
Also, the different mental images must induce brain states
easy enough to distinguish between each other.
These images are expected to produce some activity at different bandpower
and/or in different areas of  the brain.
This is why these mental images used are typically not about imagining objects,
but rather about imagining tasks
For example, \textbf{motor imagery} tasks, where the user can be asked for example to
\textit{imagine moving his right hand},
are massively used
(because large parts of the brain are allocated to body movement control
and the control of different body parts activates different brain areas).
Also, tasks like mental calculation or mental rotation of an imagined object are used.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{illustrations/cybathlon.png}
    \caption[Cybathlon game]{Cybathlon game. The patient controls a video game avatar
        using a mental-imagery based \acrshort{bci}.
        On this picture, the patient is training for the cybathlon \acrshort{bci} race.
        Source:~\cite{lotte2019inria}.}
    \label{fig:cybathlon}
\end{figure}



\subsection{Event Related Potentials}

An \textbf{\acrfull{erp}} is the measured brain response
that is the direct result of a specific sensory, cognitive,
or motor event~\cite{luck2014introduction}.
The stimuli that can elicit \acrshort{erp}s may be  visual, tactile, auditory, olfactory, gustatory, etc.
This response is electrophysiological and can be measured by \acrshort{eeg}.
When measuring them via \acrshort{meg}, we talk about \acrfull{erf}.
A typical \acrshort{erp} response is illustrated in Figure~\ref{fig:componentsofERP}.
We observe that this response contains different components.
For example, the \textbf{P300} is a characteristic one
because of its amplitude and consistency.
It occurs around 300ms after the stimulus, hence its name.
These components can be used to construct \acrshort{bci}s.

\begin{figure}
    \centering
    \includegraphics[width=.4\textwidth]{illustrations/ComponentsofERP.png}
    \caption[\acrshort{erp} components]{A waveform showing several \acrshort{erp} components,
    including the N100 (labeled N1) and P300 (labeled P3). Source:~\cite{wiki:ComponentsofERP}}
    \label{fig:componentsofERP}
\end{figure}

\textbf{\acrshort{erp} Spellers} make use of these component to allow subjects to type texts,
letter by letter.
Their setup consist in a screen displaying the alphabet in a grid
and an \acrshort{eeg} cap recording in real time the subject's brain activity.
To type, the user must first focus on the letter he wants to type.
Then, the screen will first flash a subset of the letters
and the elicited \acrshort{erp} response is observed via the \acrshort{eeg} cap.
The key is that the amplitude of the ERP components
vary with the relevance of the eliciting event -
ie: if the letter the user is focusing on flashes, the induced P300's amplitude is greater
than if some other letters flash.
So the signal containing the \acrshort{erp} can be classified into target and non-target
by machine learning models
and by repeating this process with different letter subsets,
the user's letter can be revealed.
In Figure~\ref{fig:p300}, we can observe a subject using a \acrshort{erp} speller.


\begin{figure}
    \centering
    \includegraphics[width=.6\linewidth]{illustrations/p300_left.jpg}
    \caption[ERP speller]{\acrshort{erp} speller. A keyboard is displayed on the screen and subsets of the letters are flashing intermittently.
    The subject spells words by focusing on the letter he wants to type until he sees it flashing.
    The flashing of his current letter triggers an \acrshort{erp} in his brain that is detected in real time.
    Source:~\cite{guy2018brain}.}
    \label{fig:p300}
\end{figure}


==> content_report/preamble_arpe_report.tex <==

This document is divided into main two parts.
The Chapter~\ref{chap:prereq} is an introduction to neuroscience and
brain-computer interfaces.
It is intended for the computer scientist readers
and is supposed to provide the knowledge needed
to understand our work.
%%
The Chapter~\ref{chap:article} reports the work we conducted
and is constructed as a stand-alone research article.
However it is still in construction so it has not been published yet.
The version presented in Chapter~\ref{chap:article} is actually
the first draft of this article and have not been yet reviewed by my supervisors
(due to the holidays schedules).
Please keep that in mind while reading this document.
Also, in the discussions of Section~\ref{sec:discussion},
we list some interesting leads in order to continue the development of this project.
We want to explore those leads in a PhD with Michael Tangermann
and potentially co-supervised by Théodore Papadopoulo  at the Donders Institute.


==> content_report/title_arpe_report.tex <==

\begin{titlingpage}
\begin{SingleSpace}
% \calccentering{\unitlength}
% \begin{adjustwidth*}{\unitlength}{-\unitlength}
\vspace*{35mm}
\begin{center}
\textsc{\Large ARPE report}\\[0.5cm]
\rule[0.5ex]{\linewidth}{2pt}\vspace*{-\baselineskip}\vspace*{3.2pt}
\rule[0.5ex]{\linewidth}{1pt}\\[\baselineskip]
{\HUGE Embeddings for EEG signals}\\[4mm]
{} % {\Large \textit{Effects of spatial microscopic defects on luminescence intensity}}\\
\rule[0.5ex]{\linewidth}{1pt}\vspace*{-\baselineskip}\vspace{3.2pt}
\rule[0.5ex]{\linewidth}{2pt}\\
\vspace{13mm}
\begin{centering}
\emph{Author:}\\
Pierre \textsc{Guetschel}\\[5mm]
\emph{Supervisors:} \\
Theodore \textsc{Papadopoulo} \\
Michael \textsc{Tangermann}
\end{centering}
\\[2.5cm]

\vspace{10mm}
\begin{centering}
\begin{minipage}{0.95\textwidth}
\raisebox{-0.5\height}{\includegraphics[width=0.25\textwidth]{logos/ENSPS-logo.png}} \hfill
\raisebox{-0.5\height}{\includegraphics[width=0.25\textwidth]{logos/inria-logo.png}} \hfill
\raisebox{-0.5\height}{\includegraphics[width=0.25\textwidth]{logos/donders_logo.jpg}} \hfill
\end{minipage}
\end{centering}\\
\vspace{10mm}

%{\large ATHENA Team\\
%\textsc{INRIA Sophia Antipolis}}\\
%\vspace{5mm}

\begin{minipage}{10cm}
A dissertation submitted to the \acrshort{ens} Paris Saclay in accordance with the requirements of the \textsc{\acrshort{arpe}} (\acrlong{arpe}).
\end{minipage}\\
\vspace{10mm}
{\centering\large\textsc{August 2021}}
\end{center}
%\begin{flushright}
%{\small Word count: ten thousand and four}
%\end{flushright}
% \end{adjustwidth*}
\end{SingleSpace}
\end{titlingpage}


==> frontmatter/style_arpe_report.tex <==
% Sets numbering division level
\setsecnumdepth{subsection}
\maxsecnumdepth{subsubsection}
%
% Chapter style (taken and slightly modified from Lars Madsen Memoir Chapter
% Styles document
\usepackage{calc,soul}
\makeatletter
\newlength\dlf@normtxtw
\setlength\dlf@normtxtw{\textwidth}
\newsavebox{\feline@chapter}
\newcommand\feline@chapter@marker[1][4cm]{%
	\sbox\feline@chapter{%
		\resizebox{!}{#1}{\fboxsep=1pt%
			\colorbox{gray}{\color{white}\thechapter}%
		}}%
		\rotatebox{90}{%
			\resizebox{%
				\heightof{\usebox{\feline@chapter}}+\depthof{\usebox{\feline@chapter}}}%
			{!}{\scshape\so\@chapapp}}\quad%
		\raisebox{\depthof{\usebox{\feline@chapter}}}{\usebox{\feline@chapter}}%
}
\newcommand\feline@chm[1][4cm]{%
	\sbox\feline@chapter{\feline@chapter@marker[#1]}%
	\makebox[0pt][c]{% aka \rlap
		\makebox[1cm][r]{\usebox\feline@chapter}%
	}}
\makechapterstyle{daleifmodif}{
	\renewcommand\chapnamefont{\normalfont\Large\scshape\raggedleft\so}
	\renewcommand\chaptitlefont{\normalfont\Large\bfseries\scshape}
	\renewcommand\chapternamenum{} \renewcommand\printchaptername{}
	\renewcommand\printchapternum{\null\hfill\feline@chm[2.5cm]\par}
	\renewcommand\afterchapternum{\par\vskip\midchapskip}
	\renewcommand\printchaptertitle[1]{\color{gray}\chaptitlefont\raggedleft ##1\par}
}
\makeatother
\chapterstyle{daleifmodif}

% My caption style
\newcommand{\mycaption}[2][\@empty]{
	\captionnamefont{\scshape}
	\changecaptionwidth
	\captionwidth{0.9\linewidth}
	\captiondelim{.\:}
	\indentcaption{0.75cm}
	\captionstyle[\centering]{}
	\setlength{\belowcaptionskip}{10pt}
	\ifx \@empty#1 \caption{#2}\else \caption[#1]{#2}
}
%
% My subcaption style
\newcommand{\mysubcaption}[2][\@empty]{
	\subcaptionsize{\small}
	\hangsubcaption
	\subcaptionlabelfont{\rmfamily}
	\sidecapstyle{\raggedright}
	\setlength{\belowcaptionskip}{10pt}
	\ifx \@empty#1 \subcaption{#2}\else \subcaption[#1]{#2}
}
%


==> inkscape_tex/formula_triplet_loss.tex <==
\[
    \loss^{\text{tri}}_\alpha(\tripletsindices, \vectorset) \eqdef
    \sum_{(\anchor, \positive, \negative)\in\tripletsindices}
    \maxzero{\norm{\vectora-\vectorp}-\norm{\vectora-\vectorn}+\alpha}
\]


==> inkscape_tex/hasse_lexi.tex <==
\begin{tikzpicture}[auto, x=1cm, y=.9cm]
  \node (X11)[rrec] at (0,3) {$1,1$};
  \node (X00)[rrec] at (0,0) {$0,0$};
  \node (X01)[rrec] at (0,2) {$0,1$};
  \node (X10)[rrec] at (0,1) {$1,0$};
  \draw[rel] (X11) -- (X01);
  \draw[rel] (X01) -- (X10);
  \draw[rel] (X10) -- (X00);
\end{tikzpicture}


==> inkscape_tex/hasse_prod.tex <==
\begin{tikzpicture}[auto, x=1cm, y=.9cm]
  \node (X11)[rrec] at (0,3) {$1,1$};
  \node (X00)[rrec] at (0,0) {$0,0$};
  \node (X10)[rrec] at (-.6,1.5) {$1,0$};
  \node (X01)[rrec] at (.6,1.5) {$0,1$};
  \draw[rel] (X11) -- (X10);
  \draw[rel] (X11) -- (X01);
  \draw[rel] (X00) -- (X10);
  \draw[rel] (X00) -- (X01);
\end{tikzpicture}


==> inkscape_tex/preamble.tex <==
\usepackage{tikz}						%geometric/algebraic description.
\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{mathrsfs}       % blackboard math symbols
\usepackage{stmaryrd}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% definitions %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{positioning,
               arrows,shapes,snakes,
		       automata,backgrounds,
		       petri,topaths}				%To use diverse features from tikz


%% tikz params %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \tikzstyle{every node}=[
%     draw=black, rounded corners, text centered, node distance=1.5cm,
%     minimum width=.6cm, minimum height=.6cm]

\tikzstyle{every draw}=[thick]

\tikzset{
    dotCircle/.style={circle, draw, thick, fill, inner sep=2pt},
    dotSquare/.style={draw, thick, fill, inner sep=2.5pt},
    dotDiamond/.style={draw, rotate=45, thick, fill, inner sep=2.5pt},
    rrec/.style={draw=black, rounded corners, text centered, node distance=1.5cm,
        minimum width=.6cm, minimum height=.6cm, thick},
    border/.style={dash pattern=on 3pt off 3pt, color=gray!70, thin},
    dist/.style={dash pattern=on 10pt off 2pt, thin},
    rel/.style={},
}


%% math definitions %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\anchor}{\mathrm{a}}
\newcommand{\positive}{\mathrm{p}}
\newcommand{\negative}{\mathrm{n}}
\newcommand{\rpz}{\mathnormal{f}}
\newcommand{\example}[1]{x_{#1}}
\newcommand{\embedvector}[1]{v_{#1}}

\newcommand{\exampleset}{\mathcal{X}}
\newcommand{\vectorset}{\mathcal{V}_\rpz}
\newcommand{\indices}[2]{\mathcal{I}_{#1}^{#2}}
\newcommand{\tripletsindices}{\mathcal{T}}
\newcommand{\distsymbol}{\mathnormal{d}}

\newcommand{\examplea}{\example{\anchor}}
\newcommand{\examplep}{\example{\positive}}
\newcommand{\examplen}{\example{\negative}}
\newcommand{\vectora}{\embedvector{\anchor}}
\newcommand{\vectorp}{\embedvector{\positive}}
\newcommand{\vectorn}{\embedvector{\negative}}
\newcommand{\indicesa}[1]{\indices{\anchor}{#1}}

\newcommand{\rawdist}[2]{\distsymbol\big(#1,#2\big)}

\newcommand{\vdist}[2]{\rawdist{\embedvector{#1}}{\embedvector{#2}}}
\newcommand{\vdista}[1]{\vdist{\anchor}{#1}}
\newcommand{\vdistap}{\vdista{\positive}}
\newcommand{\vdistan}{\vdista{\negative}}

\newcommand{\longdist}[2]{\rawdist{\rpz(#1)}{\rpz(#2)}}
\newcommand{\dist}[2]{\distsymbol_{\rpz #1}(#2)}
\newcommand{\longdista} [1]{\longdist{\anchor}  {#1}}
\newcommand{\longdistai}[1]{\longdist{\anchor_i}{#1}}
\newcommand{\dista} [1]{\dist{\anchor}  {#1}}
\newcommand{\distai}[1]{\dist{\anchor_i}{#1}}

\newcommand{\maxzero}[1]{\left[ #1 \right]_+}
\newcommand{\subjectt}{ \texttt{subject} }
\newcommand{\targett}{ \texttt{im\_class} }
%\newcommand{\targett}{ \texttt{target} }
\newcommand{\eqdef}{\buildrel \text{\tiny def}\over =}
\newcommand{\loss}{\mathscr{L}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\intset}[1]{\llbracket #1 \rrbracket}


==> inkscape_tex/space_ladder_loss.tex <==
\begin{tikzpicture}[x=0.8cm,y=0.8cm]
  \node (anchor)[dotCircle, fill=blue] at (0,0) [label=left:$\vectora$]  {};
  \node (X1)[dotDiamond, fill=green] at (.3,1.3) [label=left:$\embedvector{i_1}$]  {};
  \node (X2)[dotDiamond, fill=orange] at (3,0) [label=above:$\embedvector{i_2}$]  {};
  \node (X3)[dotDiamond, fill=red] at (3.5,3.5) [label=$\embedvector{i_3}$]  {};
  \draw[dist] (anchor) -- (X1);
  \draw[dist] (anchor) -- (X2);
  \draw[dist] (anchor) -- (X3);
  \draw[border] (0,1.7) arc (90:-40:1.7)  ;
  \draw[border] (0,2.5) arc (90:-40:2.5)  ;
  \draw[border] (0,3.5) arc (90:-40:3.5)  ;
  \draw[border] (0,4.3) arc (90:-40:4.3)  ;
  \draw[dist,<->] (1.4722, -0.85) -- (2.1651,-1.25)node[midway,above,draw=none] {$\alpha_1$};
  \draw[dist,<->] (3.0311, -1.75) -- (3.7239,-2.15)node[midway,above,draw=none] {$\alpha_2$};
\end{tikzpicture}


==> inkscape_tex/space_triplet_loss.tex <==
\begin{tikzpicture}[x=0.8cm,y=0.8cm]
  \node (anchor)[dotCircle, fill=blue] at (0,0) [label=left:$\vectora$]  {};
  \node (pos)[dotDiamond, fill=green] at (2.3,.4) [label=right:$\vectorp$]  {};
  \node (neg)[dotSquare, fill=red] at (3,3) [label=$\vectorn$]  {};
  \draw[dist] (anchor) -- (pos) node[midway,below,draw=none,sloped] {$\vdistap$};
  \draw[dist] (anchor) -- (neg) node[midway,above,draw=none,sloped] {$\vdistan$};
  \draw[border] (0,3.7) arc (90:-40:3.7)  ;
  \draw[border] (0,2.7) arc (90:-40:2.7)  ;
  \draw[dist,<->] (2.33827, -1.35) -- (3.2043,-1.85)node[midway,above,draw=none] {$\alpha$};
\end{tikzpicture}

